Learning Implicit Priors for Motion Optimization

In this paper, we focus on the problem of integrating Energy-based Models (EBM) as guiding priors for motion optimization. EBMs are a set of neural networks that can represent expressive probability density distributions in terms of a Gibbs distribution parameterized by a suitable energy function. Due to their implicit nature, they can easily be integrated as optimization factors or as initial sampling distributions in the motion optimization problem, making them good candidates to integrate data-driven priors in the motion optimization problem. In this work, we present a set of required modeling and algorithmic choices to adapt EBMs into motion optimization. We investigate the benefit of including additional regularizers in the learning of the EBMs to use them with gradient-based optimizers and we present a set of EBM architectures to learn generalizable distributions for manipulation tasks. We present multiple cases in which the EBM could be integrated for motion optimization and evaluate the performance of learned EBMs as guiding priors for both simulated and real robot experiments.

==> exps/pouring_results.tex <==
\resizebox{0.4999\textwidth}{!}{
	\begin{tabular}{l|c|c|c|c } 
		 & No priors & traj. \gls{ebm} + reg~\eqref{eq:dsm} & phase \gls{ebm}  & phase \gls{ebm} + reg.~\eqref{eq:dsm}\\
		 \hline
		 No obst. & $0.96$  & $0.94$  & $0.9$ &  $\mathbf{1.}$ \\
		 \hline
		 Obst. & $0.52$  &  $0.5$  & $0.7$  &  $\mathbf{0.86}$ \\
		\hline
	\end{tabular}}


==> sections/reorganize.tex <==
\subsection{An written}

In this work, we focus on the robotics manipulation settings, where the motion optimization objectives has to incorporate multiple task objectives and constraints, to achieve sequence of object-centric manipulations. Motivated by a general theoretical framework to introduce inductive bias into the planning problem, we adopt the perspective of planning as inference similar to ~\cite{mukadam2018continuous, sodhi2021leo}, where the
planning problem is framed as maximum a posteriori (MAP) trajectory given multiple priors over trajectories and a likelihood of events of interest that the trajectory must satisfy.

The events of interest can be represented by a set of $K$ chosen task context variables $\mathcal{E} = \{\ve_k\}_{k=1}^K$, such as the poses of the object of interest, target placement poses for pick and place task, target cup pose for pouring task, etc. Without the loss of generality, the posterior over the trajectory $\tau, \vs_t \equiv \tau_t $ can be defined as a factor graph of \textit{unconditional} and \textit{conditional} energy functions depending on the context variables:

\begin{align}
\label{eq:traj_posterior}
   P(\tau | \mathcal{E}) &= \frac{1}{Z(\tau; \mathcal{E})} \exp [- \boldsymbol{E}(\tau; \mathcal{E})]\\
                         &= \frac{1}{Z(\tau; \mathcal{E})} \exp [- \sum_{k}\boldsymbol{E}_k(\tau; \ve_k) - \sum_{n}\boldsymbol{E}_n(\tau)] \nonumber
\end{align}
where the conditional energy function $\boldsymbol{E}_k$ represents the introduced bias as implicits priors and the unconditional energy function $\boldsymbol{E}_n$ represents trajectory instrinsic factors such as smoothness factor, starting cost factor, final cost factor etc. and $Z(\tau; \mathcal{E}) = \int_{\tau} \exp [- \boldsymbol{E}(\tau; \mathcal{E})] d\tau$ is the partition function to normalize the distribution.

Then, the optimal trajectory can be inferred by performing MAP over the log posterior $P(\tau | \mathcal{E})$:

\begin{align}
\label{eq:map_posterior}
\tau^*_{1:T} &= \arg \max \log P(\tau | \mathcal{E}) \\
             &= \arg \max \log Z(\tau; \mathcal{E})\exp [- \sum_{k}\boldsymbol{E}_k(\tau; \ve_k) - \sum_{n}\boldsymbol{E}_n(\tau)] \nonumber\\
             &= \arg \min \sum_{k}\boldsymbol{E}_k(\tau; \ve_k) + \sum_{n}\boldsymbol{E}_n(\tau) \nonumber\\
\end{align}

As expected, the equation \eqref{eq:map_posterior} is the general form of the trajectory optimization problem in \eqref{eq:traj_opt}, where we additionally introduce task-dependent implicits priors as conditional energy functions $\{\boldsymbol{E}_k(\tau; \ve_k)\}$.

\subsection{Implicit Priors for Motion Optimization}

Note (An): maybe we can talk about instead of realizing the (un)conditional energy function as simple Gaussian like previous works, we say we adopt a more powerful multi-modal representation by defining the (un)conditional energy function as EBMs. Maybe make clear that on the cost factor part:
\begin{enumerate}
    \item for \gls{sgpmp}, we clearly introduce the "standard" Gaussian factors as standard costs (like previous works)
    \item our novel ideas: learn modular EBMs and superposition together with previous standard costs.
\end{enumerate}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

